Early-Excess SNe Ia Show Strong C II Absorption

Some type Ia supernovae (SNe Ia) exhibit an early excess in their rising light curves, but the physical origin of this behavior remains uncertain. The processes driving these excesses affect the ejecta at early times and may also imprint on the outermost layers. We investigate whether early excesses are associated with differences in unburned material by measuring pre-maximum carbon absorption. Using multi-component Gaussian fits to the blended Si II $\lambda6355$ and C II $\lambda6580$ region, we measure pseudo-equivalent widths and velocities for a sample of 35 nonpeculiar SNe Ia with rising light curve categorizations. We find that early-excess objects ($n=13$) tend to exhibit stronger C II absorption than non-excesses ($n=22$) at phases earlier than approximately $-13$ d, with a two-sample K-S test of the earliest measurements yielding $p=0.025$. In contrast, the HV Si II components do not clearly separate the two groups. Early-excess SNe Ia tend to be more luminous and decline more slowly, but objects with similar maximum-light properties span a range of C II pseudo-equivalent widths, suggesting that this effect is distinct from the known luminosity-width relation. We show that, at least in some cases, when objects have similar light-curve shape and photospheric temperature, the effect we see is not driven by ionization but by distinct differences in the explosion, such as carbon abundance and density and the efficiency of burning in the WD. Our results provide a new constraint on SN Ia explosion models for early excesses, as they must produce a tendency for stronger early C II absorption.

==> tables/measurements_table_full.tex <==
\begin{table*}[ht]
\centering
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.25}
\caption{Spectroscopic measurements for the \ion{C}{2} $\lambda6580$, \ion{Si}{2} $\lambda6355$, and high-velocity \ion{Si}{2} $\lambda6355$ absorption features. Phase is calculated relative to $B$-band maximum light in the rest frame. Positive and negative uncertainties are listed in separate columns. When carbon is undetectable, C pEW is computed from the $3\sigma$ upper-bound with a corresponding $1\sigma$ uncertainty using $W_{line} = 50$ for the C II Gaussian (equation 5).}
\label{tab:pew_measurements_full}
\begin{tabular}{llcccccccc}
\hline
\shortstack{\strut Object} & \shortstack{\strut Component} & \shortstack{\strut MJD} & \shortstack{\strut Phase \\ (days)} & \shortstack{\strut pEW \\ (Å)} & \shortstack{\strut $+\sigma_{\rm pEW}$ \\ (Å)} & \shortstack{\strut $-\sigma_{\rm pEW}$ \\ (Å)} & \shortstack{\strut Velocity \\ ($\mathrm{km~s^{-1}}$)} & \shortstack{\strut $+\sigma_v$ \\ ($\mathrm{km~s^{-1}}$)} & \shortstack{\strut $-\sigma_v$ \\ ($\mathrm{km~s^{-1}}$)} \\
\hline
SN\,2009ig & C & $55065.0$ & $-14.9$ & $1.080$ & $0.528$ & $0.438$ & $17090$ & $691$ & $192$ \\
SN\,2009ig & Si & $55065.0$ & $-14.9$ & $108.378$ & $12.096$ & $15.617$ & $18207$ & $405$ & $543$ \\
SN\,2009ig & HV Si & $55065.0$ & $-14.9$ & $70.755$ & $13.760$ & $10.636$ & $24240$ & $144$ & $262$ \\
SN\,2009ig & C & $55065.6$ & $-14.3$ & $0.539$ & $0.181$ & $0.321$ & $16746$ & $75$ & $66$ \\
SN\,2009ig & Si & $55065.6$ & $-14.3$ & $123.833$ & $5.583$ & $15.433$ & $18652$ & $156$ & $458$ \\
SN\,2009ig & HV Si & $55065.6$ & $-14.3$ & $60.203$ & $12.467$ & $4.265$ & $24410$ & $46$ & $151$ \\
SN\,2009ig & C & $55066.6$ & $-13.3$ & $0.116$ & $0.178$ & $0.083$ & $16388$ & $1256$ & $256$ \\
SN\,2009ig & Si & $55066.6$ & $-13.3$ & $115.372$ & $7.386$ & $10.766$ & $17663$ & $216$ & $312$ \\
SN\,2009ig & HV Si & $55066.6$ & $-13.3$ & $50.550$ & $7.933$ & $5.615$ & $23613$ & $75$ & $139$ \\
SN\,2009ig & C & $55067.0$ & $-12.9$ & $0.079$ & $0.053$ & $0.062$ & $16216$ & $61$ & $66$ \\
SN\,2009ig & Si & $55067.0$ & $-12.9$ & $108.835$ & $4.260$ & $7.288$ & $17109$ & $117$ & $205$ \\
SN\,2009ig & HV Si & $55067.0$ & $-12.9$ & $33.200$ & $4.897$ & $2.861$ & $23203$ & $56$ & $79$ \\
SN\,2009ig & C & $55068.5$ & $-11.4$ & $0.090$ & $0.030$ & $0.030$ & \nodata & \nodata & \nodata \\
SN\,2009ig & Si & $55068.5$ & $-11.4$ & $89.956$ & $5.557$ & $9.323$ & $16148$ & $54$ & $96$ \\
SN\,2009ig & HV Si & $55068.5$ & $-11.4$ & $20.762$ & $3.086$ & $3.010$ & $22664$ & $89$ & $280$ \\
SN\,2009ig & C & $55070.5$ & $-9.4$ & $0.100$ & $0.033$ & $0.033$ & \nodata & \nodata & \nodata \\
SN\,2009ig & Si & $55070.5$ & $-9.4$ & $77.736$ & $1.546$ & $4.828$ & $14568$ & $22$ & $25$ \\
SN\,2009ig & HV Si & $55070.5$ & $-9.4$ & $9.120$ & $0.547$ & $1.628$ & $21966$ & $65$ & $187$ \\
SN\,2009ig & C & $55071.5$ & $-8.4$ & $0.195$ & $0.065$ & $0.065$ & \nodata & \nodata & \nodata \\
SN\,2009ig & Si & $55071.5$ & $-8.4$ & $83.416$ & $3.567$ & $7.863$ & $14417$ & $33$ & $52$ \\
SN\,2009ig & HV Si & $55071.5$ & $-8.4$ & $4.260$ & $1.276$ & $1.539$ & $21465$ & $126$ & $230$ \\
SN\,2009ig & Si & $55079.0$ & $-1.0$ & $80.274$ & $0.803$ & $4.120$ & $13236$ & $59$ & $10$ \\
SN\,2011fe & C & $55798.0$ & $-16.5$ & $7.205$ & $1.545$ & $1.347$ & $13225$ & $91$ & $87$ \\
SN\,2011fe & Si & $55798.0$ & $-16.5$ & $114.095$ & $1.831$ & $12.063$ & $14526$ & $23$ & $75$ \\
SN\,2011fe & C & $55799.0$ & $-15.5$ & $0.991$ & $0.637$ & $0.789$ & $12822$ & $141$ & $207$ \\
SN\,2011fe & Si & $55799.0$ & $-15.5$ & $97.913$ & $3.548$ & $17.189$ & $13916$ & $58$ & $130$ \\
SN\,2011fe & C & $55800.0$ & $-14.5$ & $0.264$ & $0.856$ & $0.217$ & $12499$ & $352$ & $367$ \\
SN\,2011fe & Si & $55800.0$ & $-14.5$ & $101.043$ & $5.297$ & $18.522$ & $13212$ & $37$ & $93$ \\
SN\,2011fe & C & $55801.0$ & $-13.5$ & $0.449$ & $0.680$ & $0.386$ & $11672$ & $477$ & $190$ \\
SN\,2011fe & Si & $55801.0$ & $-13.5$ & $102.170$ & $2.925$ & $6.649$ & $12479$ & $32$ & $60$ \\
SN\,2011fe & C & $55803.0$ & $-11.5$ & $1.485$ & $0.863$ & $1.130$ & $11558$ & $79$ & $66$ \\
SN\,2011fe & Si & $55803.0$ & $-11.5$ & $95.235$ & $3.235$ & $9.171$ & $11729$ & $40$ & $68$ \\
SN\,2011fe & C & $55804.0$ & $-10.5$ & $1.001$ & $0.732$ & $0.803$ & $11266$ & $42$ & $62$ \\
SN\,2011fe & Si & $55804.0$ & $-10.5$ & $94.895$ & $3.020$ & $5.565$ & $11439$ & $31$ & $50$ \\
SN\,2011fe & C & $55805.2$ & $-9.3$ & $1.195$ & $0.664$ & $1.157$ & $11067$ & $112$ & $61$ \\
SN\,2011fe & Si & $55805.2$ & $-9.3$ & $88.341$ & $2.609$ & $5.030$ & $11230$ & $34$ & $41$ \\
SN\,2011fe & C & $55806.2$ & $-8.3$ & $1.007$ & $0.761$ & $0.982$ & $10904$ & $37$ & $70$ \\
SN\,2011fe & Si & $55806.2$ & $-8.3$ & $85.793$ & $2.705$ & $4.571$ & $10987$ & $33$ & $37$ \\
SN\,2011fe & C & $55807.3$ & $-7.2$ & $0.600$ & $0.669$ & $0.573$ & $10595$ & $48$ & $114$ \\
SN\,2011fe & Si & $55807.3$ & $-7.2$ & $85.001$ & $2.427$ & $5.432$ & $10823$ & $27$ & $42$ \\
SN\,2011fe & C & $55808.2$ & $-6.3$ & $0.290$ & $0.636$ & $0.267$ & $10374$ & $38$ & $57$ \\
SN\,2011fe & Si & $55808.2$ & $-6.3$ & $83.762$ & $2.416$ & $5.512$ & $10671$ & $29$ & $42$ \\
SN\,2011fe & C & $55809.2$ & $-5.3$ & $0.227$ & $0.506$ & $0.215$ & $10175$ & $37$ & $45$ \\
SN\,2011fe & Si & $55809.2$ & $-5.3$ & $85.915$ & $1.611$ & $2.085$ & $10595$ & $19$ & $18$ \\
SN\,2011fe & Si & $55812.0$ & $-2.5$ & $93.431$ & $2.969$ & $4.085$ & $10278$ & $29$ & $31$ \\
SN\,2011fe & C & $55812.0$ & $-2.5$ & $0.052$ & $0.344$ & $0.050$ & $9814$ & $252$ & $630$ \\
SN\,2011fe & Si & $55813.0$ & $-1.5$ & $96.637$ & $1.745$ & $2.088$ & $10339$ & $22$ & $18$ \\
SN\,2011fe & C & $55813.0$ & $-1.5$ & $0.046$ & $0.309$ & $0.045$ & $9804$ & $233$ & $557$ \\
SN\,2011fe & Si & $55814.2$ & $-0.3$ & $94.880$ & $2.071$ & $3.989$ & $10136$ & $44$ & $23$ \\
SN\,2011fe & C & $55814.2$ & $-0.3$ & $0.041$ & $0.267$ & $0.036$ & $9585$ & $380$ & $401$ \\
LSQ12gdj & C & $56244.1$ & $-8.2$ & $0.812$ & $0.271$ & $0.271$ & \nodata & \nodata & \nodata \\
LSQ12gdj & Si & $56244.1$ & $-8.2$ & $9.644$ & $1.960$ & $2.136$ & $9640$ & $244$ & $254$ \\
LSQ12gdj & C & $56246.1$ & $-6.2$ & $0.332$ & $0.111$ & $0.111$ & \nodata & \nodata & \nodata \\
LSQ12gdj & Si & $56246.1$ & $-6.2$ & $21.770$ & $0.996$ & $2.622$ & $10125$ & $88$ & $155$ \\
LSQ12gdj & C & $56250.0$ & $-2.4$ & $0.516$ & $0.172$ & $0.172$ & \nodata & \nodata & \nodata \\
LSQ12gdj & Si & $56250.0$ & $-2.4$ & $33.758$ & $1.819$ & $1.809$ & $10489$ & $87$ & $86$ \\
LSQ12gdj & C & $56251.0$ & $-1.5$ & $0.429$ & $0.143$ & $0.143$ & \nodata & \nodata & \nodata \\
LSQ12gdj & Si & $56251.0$ & $-1.5$ & $35.753$ & $1.741$ & $2.372$ & $10601$ & $97$ & $61$ \\
SN\,2012cg & C & $56065.0$ & $-16.3$ & $54.868$ & $3.702$ & $4.302$ & $18997$ & $182$ & $197$ \\
SN\,2012cg & Si & $56065.0$ & $-16.3$ & $50.702$ & $4.309$ & $5.651$ & $19484$ & $292$ & $316$ \\
SN\,2012cg & C & $56066.0$ & $-15.3$ & $24.846$ & $2.590$ & $2.321$ & $15967$ & $966$ & $435$ \\
SN\,2012cg & Si & $56066.0$ & $-15.3$ & $73.665$ & $7.217$ & $13.881$ & $16071$ & $93$ & $91$ \\
SN\,2012cg & HV Si & $56066.0$ & $-15.3$ & $17.214$ & $0.693$ & $0.826$ & $21115$ & $117$ & $282$ \\
SN\,2012cg & C & $56067.0$ & $-14.3$ & $5.581$ & $1.065$ & $0.768$ & $13783$ & $36$ & $37$ \\
SN\,2012cg & Si & $56067.0$ & $-14.3$ & $84.486$ & $2.998$ & $9.809$ & $14265$ & $103$ & $258$ \\
SN\,2012cg & HV Si & $56067.0$ & $-14.3$ & $19.073$ & $1.407$ & $1.154$ & $19109$ & $131$ & $406$ \\
SN\,2012cg & C & $56068.0$ & $-13.3$ & $1.512$ & $0.756$ & $0.806$ & $12943$ & $114$ & $111$ \\
SN\,2012cg & Si & $56068.0$ & $-13.3$ & $71.994$ & $3.653$ & $6.752$ & $13265$ & $105$ & $190$ \\
SN\,2012cg & HV Si & $56068.0$ & $-13.3$ & $22.669$ & $4.887$ & $2.863$ & $18796$ & $148$ & $297$ \\
SN\,2012cg & C & $56072.0$ & $-9.3$ & $0.277$ & $0.424$ & $0.219$ & $13103$ & $88$ & $115$ \\
SN\,2012cg & Si & $56072.0$ & $-9.3$ & $19.776$ & $2.551$ & $3.590$ & $11280$ & $29$ & $83$ \\
SN\,2012cg & HV Si & $56072.0$ & $-9.3$ & $2.085$ & $3.175$ & $1.323$ & $15491$ & $970$ & $697$ \\
SN\,2012cg & C & $56075.0$ & $-6.3$ & $0.110$ & $0.037$ & $0.037$ & \nodata & \nodata & \nodata \\
SN\,2012cg & Si & $56075.0$ & $-6.3$ & $45.053$ & $4.411$ & $6.327$ & $10668$ & $104$ & $128$ \\
SN\,2012cg & C & $56076.0$ & $-5.3$ & $0.077$ & $0.026$ & $0.026$ & \nodata & \nodata & \nodata \\
SN\,2012cg & Si & $56076.0$ & $-5.3$ & $49.271$ & $3.990$ & $6.730$ & $10550$ & $118$ & $101$ \\
SN\,2012cg & C & $56079.0$ & $-2.3$ & $0.190$ & $0.063$ & $0.063$ & \nodata & \nodata & \nodata \\
SN\,2012cg & Si & $56079.0$ & $-2.3$ & $61.512$ & $3.851$ & $5.760$ & $10267$ & $73$ & $79$ \\
SN\,2012fr & C & $56230.5$ & $-12.0$ & $0.667$ & $0.835$ & $0.564$ & $14581$ & $204$ & $152$ \\
SN\,2012fr & Si & $56230.5$ & $-12.0$ & $18.097$ & $2.872$ & $2.682$ & $12787$ & $222$ & $209$ \\
SN\,2012fr & HV Si & $56230.5$ & $-12.0$ & $136.396$ & $4.097$ & $4.837$ & $21376$ & $53$ & $43$ \\
SN\,2012fr & C & $56231.5$ & $-11.0$ & $0.270$ & $0.496$ & $0.201$ & $14553$ & $154$ & $165$ \\
SN\,2012fr & Si & $56231.5$ & $-11.0$ & $23.431$ & $2.464$ & $2.441$ & $12526$ & $147$ & $161$ \\
SN\,2012fr & HV Si & $56231.5$ & $-11.0$ & $105.226$ & $4.542$ & $3.530$ & $21049$ & $49$ & $45$ \\
SN\,2012fr & C & $56233.0$ & $-9.5$ & $0.249$ & $0.178$ & $0.125$ & $15235$ & $38$ & $47$ \\
SN\,2012fr & Si & $56233.0$ & $-9.5$ & $37.710$ & $3.088$ & $3.536$ & $12990$ & $127$ & $134$ \\
SN\,2012fr & HV Si & $56233.0$ & $-9.5$ & $46.605$ & $3.061$ & $3.309$ & $20777$ & $110$ & $109$ \\
SN\,2012fr & C & $56233.7$ & $-8.9$ & $0.655$ & $0.218$ & $0.218$ & \nodata & \nodata & \nodata \\
SN\,2012fr & Si & $56233.7$ & $-8.9$ & $44.418$ & $3.038$ & $3.092$ & $12757$ & $113$ & $116$ \\
SN\,2012fr & HV Si & $56233.7$ & $-8.9$ & $36.751$ & $3.245$ & $3.869$ & $20442$ & $148$ & $150$ \\
SN\,2012fr & C & $56235.0$ & $-7.6$ & $0.187$ & $0.062$ & $0.062$ & \nodata & \nodata & \nodata \\
SN\,2012fr & Si & $56235.0$ & $-7.6$ & $50.756$ & $1.875$ & $3.276$ & $12454$ & $24$ & $27$ \\
SN\,2012fr & HV Si & $56235.0$ & $-7.6$ & $18.066$ & $2.422$ & $6.156$ & $19944$ & $98$ & $231$ \\
SN\,2012fr & C & $56236.0$ & $-6.6$ & $0.124$ & $0.041$ & $0.041$ & \nodata & \nodata & \nodata \\
SN\,2012fr & Si & $56236.0$ & $-6.6$ & $53.583$ & $2.134$ & $3.099$ & $12362$ & $15$ & $15$ \\
SN\,2012fr & HV Si & $56236.0$ & $-6.6$ & $15.699$ & $2.515$ & $7.187$ & $19730$ & $166$ & $482$ \\
SN\,2012fr & C & $56237.4$ & $-5.2$ & $0.074$ & $0.025$ & $0.025$ & \nodata & \nodata & \nodata \\
SN\,2012fr & Si & $56237.4$ & $-5.2$ & $53.162$ & $2.692$ & $3.060$ & $12196$ & $9$ & $10$ \\
SN\,2012fr & HV Si & $56237.4$ & $-5.2$ & $13.228$ & $4.012$ & $6.779$ & $19699$ & $232$ & $536$ \\
SN\,2012fr & C & $56239.0$ & $-3.6$ & $0.275$ & $0.092$ & $0.092$ & \nodata & \nodata & \nodata \\
SN\,2012fr & Si & $56239.0$ & $-3.6$ & $60.778$ & $1.958$ & $5.482$ & $12199$ & $16$ & $19$ \\
SN\,2012fr & HV Si & $56239.0$ & $-3.6$ & $6.535$ & $2.190$ & $1.214$ & $18585$ & $323$ & $677$ \\
SN\,2012fr & C & $56240.0$ & $-2.6$ & $0.200$ & $0.067$ & $0.067$ & \nodata & \nodata & \nodata \\
SN\,2012fr & Si & $56240.0$ & $-2.6$ & $59.979$ & $2.495$ & $3.024$ & $12137$ & $49$ & $59$ \\
SN\,2012fr & C & $56241.0$ & $-1.6$ & $0.260$ & $0.087$ & $0.087$ & \nodata & \nodata & \nodata \\
SN\,2012fr & Si & $56241.0$ & $-1.6$ & $63.847$ & $2.483$ & $2.871$ & $12041$ & $30$ & $36$ \\
SN\,2012ht & C & $56283.0$ & $-12.6$ & $5.815$ & $2.465$ & $2.125$ & $12899$ & $78$ & $85$ \\
SN\,2012ht & Si & $56283.0$ & $-12.6$ & $58.522$ & $2.505$ & $3.556$ & $11727$ & $189$ & $177$ \\
SN\,2012ht & HV Si & $56283.0$ & $-12.6$ & $34.024$ & $3.333$ & $3.625$ & $15248$ & $122$ & $101$ \\
SN\,2012ht & C & $56284.7$ & $-10.9$ & $6.523$ & $2.983$ & $3.845$ & $13091$ & $441$ & $332$ \\
SN\,2012ht & Si & $56284.7$ & $-10.9$ & $78.459$ & $6.733$ & $11.215$ & $11970$ & $198$ & $192$ \\
SN\,2012ht & HV Si & $56284.7$ & $-10.9$ & $16.199$ & $3.058$ & $3.593$ & $15735$ & $178$ & $251$ \\
SN\,2012ht & C & $56285.7$ & $-9.9$ & $4.787$ & $4.608$ & $2.863$ & $12224$ & $577$ & $223$ \\
SN\,2012ht & Si & $56285.7$ & $-9.9$ & $88.149$ & $5.891$ & $17.022$ & $11987$ & $143$ & $137$ \\
SN\,2012ht & C & $56287.7$ & $-7.9$ & $3.879$ & $2.361$ & $2.667$ & $12144$ & $296$ & $131$ \\
SN\,2012ht & Si & $56287.7$ & $-7.9$ & $98.519$ & $3.865$ & $12.341$ & $11561$ & $114$ & $59$ \\
SN\,2012ht & C & $56288.2$ & $-7.4$ & $3.197$ & $1.794$ & $2.116$ & $11781$ & $56$ & $49$ \\
SN\,2012ht & Si & $56288.2$ & $-7.4$ & $95.841$ & $2.436$ & $6.187$ & $11526$ & $34$ & $29$ \\
SN\,2012ht & C & $56291.7$ & $-3.9$ & $0.456$ & $1.408$ & $0.397$ & $10895$ & $529$ & $356$ \\
SN\,2012ht & Si & $56291.7$ & $-3.9$ & $101.884$ & $6.607$ & $20.510$ & $10917$ & $81$ & $167$ \\
SN\,2012ht & C & $56294.3$ & $-1.3$ & $0.135$ & $0.672$ & $0.135$ & $10987$ & $620$ & $434$ \\
SN\,2012ht & Si & $56294.3$ & $-1.3$ & $112.573$ & $2.021$ & $7.787$ & $10791$ & $30$ & $37$ \\
iPTF13dge & C & $56543.3$ & $-14.5$ & $0.292$ & $0.402$ & $0.292$ & $14167$ & $643$ & $245$ \\
iPTF13dge & Si & $56543.3$ & $-14.5$ & $96.172$ & $6.482$ & $7.558$ & $13450$ & $162$ & $144$ \\
iPTF13dge & HV Si & $56543.3$ & $-14.5$ & $27.052$ & $2.783$ & $3.436$ & $17525$ & $131$ & $150$ \\
iPTF13dge & C & $56547.3$ & $-10.5$ & $0.420$ & $0.140$ & $0.140$ & \nodata & \nodata & \nodata \\
iPTF13dge & Si & $56547.3$ & $-10.5$ & $107.531$ & $1.665$ & $6.617$ & $12865$ & $26$ & $60$ \\
iPTF13dge & C & $56548.7$ & $-9.2$ & $0.353$ & $0.118$ & $0.118$ & \nodata & \nodata & \nodata \\
iPTF13dge & Si & $56548.7$ & $-9.2$ & $99.969$ & $5.473$ & $5.741$ & $12360$ & $99$ & $74$ \\
iPTF13dge & C & $56554.7$ & $-3.2$ & $0.260$ & $0.087$ & $0.087$ & \nodata & \nodata & \nodata \\
iPTF13dge & Si & $56554.7$ & $-3.2$ & $111.514$ & $1.962$ & $3.036$ & $11410$ & $26$ & $30$ \\
iPTF13ebh & C & $56611.0$ & $-11.7$ & $7.813$ & $18.466$ & $4.575$ & $15476$ & $3421$ & $852$ \\
iPTF13ebh & Si & $56611.0$ & $-11.7$ & $61.804$ & $9.391$ & $11.945$ & $12115$ & $642$ & $600$ \\
iPTF13ebh & HV Si & $56611.0$ & $-11.7$ & $18.010$ & $9.824$ & $6.511$ & $15188$ & $410$ & $399$ \\
iPTF13ebh & C & $56616.0$ & $-6.8$ & $1.016$ & $0.339$ & $0.339$ & \nodata & \nodata & \nodata \\
iPTF13ebh & Si & $56616.0$ & $-6.8$ & $114.468$ & $3.874$ & $13.881$ & $11090$ & $67$ & $101$ \\
iPTF13ebh & C & $56618.0$ & $-4.8$ & $0.582$ & $0.194$ & $0.194$ & \nodata & \nodata & \nodata \\
iPTF13ebh & Si & $56618.0$ & $-4.8$ & $120.753$ & $2.997$ & $6.771$ & $11011$ & $36$ & $44$ \\
iPTF13ebh & C & $56619.0$ & $-3.8$ & $0.261$ & $0.087$ & $0.087$ & \nodata & \nodata & \nodata \\
iPTF13ebh & Si & $56619.0$ & $-3.8$ & $123.793$ & $2.055$ & $7.835$ & $10824$ & $23$ & $50$ \\
iPTF13ebh & C & $56620.0$ & $-2.9$ & $0.429$ & $0.143$ & $0.143$ & \nodata & \nodata & \nodata \\
iPTF13ebh & Si & $56620.0$ & $-2.9$ & $122.295$ & $2.094$ & $7.235$ & $10456$ & $102$ & $36$ \\
iPTF13ebh & C & $56622.0$ & $-0.9$ & $0.215$ & $0.072$ & $0.072$ & \nodata & \nodata & \nodata \\
iPTF13ebh & Si & $56622.0$ & $-0.9$ & $123.892$ & $2.374$ & $5.427$ & $10112$ & $38$ & $57$ \\
SN\,2013dy & C & $56484.6$ & $-16.0$ & $37.256$ & $3.490$ & $4.292$ & $16641$ & $192$ & $195$ \\
SN\,2013dy & Si & $56484.6$ & $-16.0$ & $46.644$ & $6.428$ & $8.640$ & $16836$ & $211$ & $461$ \\
SN\,2013dy & HV Si & $56484.6$ & $-16.0$ & $13.911$ & $8.959$ & $3.366$ & $22652$ & $347$ & $594$ \\
SN\,2013dy & C & $56488.4$ & $-12.3$ & $0.103$ & $0.196$ & $0.082$ & $11876$ & $1322$ & $185$ \\
SN\,2013dy & Si & $56488.4$ & $-12.3$ & $53.045$ & $1.360$ & $2.329$ & $12719$ & $33$ & $55$ \\
SN\,2013dy & C & $56490.0$ & $-10.7$ & $0.115$ & $0.060$ & $0.060$ & $11850$ & $64$ & $47$ \\
SN\,2013dy & Si & $56490.0$ & $-10.7$ & $45.454$ & $3.380$ & $2.421$ & $11411$ & $88$ & $66$ \\
SN\,2013dy & C & $56491.0$ & $-9.7$ & $0.137$ & $0.046$ & $0.046$ & \nodata & \nodata & \nodata \\
SN\,2013dy & Si & $56491.0$ & $-9.7$ & $46.333$ & $2.789$ & $5.314$ & $11180$ & $83$ & $120$ \\
SN\,2013dy & C & $56493.0$ & $-7.7$ & $0.233$ & $0.078$ & $0.078$ & \nodata & \nodata & \nodata \\
SN\,2013dy & Si & $56493.0$ & $-7.7$ & $49.127$ & $3.284$ & $5.588$ & $10725$ & $74$ & $110$ \\
SN\,2013dy & C & $56494.0$ & $-6.7$ & $0.144$ & $0.048$ & $0.048$ & \nodata & \nodata & \nodata \\
SN\,2013dy & Si & $56494.0$ & $-6.7$ & $44.112$ & $3.949$ & $3.429$ & $10413$ & $91$ & $86$ \\
SN\,2013dy & C & $56497.3$ & $-3.4$ & $0.219$ & $0.073$ & $0.073$ & \nodata & \nodata & \nodata \\
SN\,2013dy & Si & $56497.3$ & $-3.4$ & $53.429$ & $1.638$ & $3.793$ & $10419$ & $90$ & $42$ \\
SN\,2013dy & C & $56500.0$ & $-0.7$ & $0.233$ & $0.078$ & $0.078$ & \nodata & \nodata & \nodata \\
SN\,2013dy & Si & $56500.0$ & $-0.7$ & $63.771$ & $2.339$ & $4.891$ & $10041$ & $65$ & $51$ \\
SN\,2013gy & C & $56633.5$ & $-14.8$ & $0.384$ & $0.128$ & $0.128$ & \nodata & \nodata & \nodata \\
SN\,2013gy & Si & $56633.5$ & $-14.8$ & $102.518$ & $2.186$ & $4.800$ & $13598$ & $100$ & $35$ \\
SN\,2013gy & C & $56634.8$ & $-13.5$ & $3.325$ & $1.108$ & $1.108$ & \nodata & \nodata & \nodata \\
SN\,2013gy & Si & $56634.8$ & $-13.5$ & $103.825$ & $6.000$ & $6.205$ & $12896$ & $123$ & $129$ \\
SN\,2013gy & C & $56635.7$ & $-12.6$ & $1.437$ & $0.479$ & $0.479$ & \nodata & \nodata & \nodata \\
SN\,2013gy & Si & $56635.7$ & $-12.6$ & $99.426$ & $4.982$ & $5.116$ & $12895$ & $71$ & $65$ \\
SN\,2013gy & C & $56640.0$ & $-8.4$ & $0.093$ & $0.031$ & $0.031$ & \nodata & \nodata & \nodata \\
SN\,2013gy & Si & $56640.0$ & $-8.4$ & $100.208$ & $3.934$ & $8.443$ & $11401$ & $80$ & $59$ \\
SN\,2013gy & C & $56641.4$ & $-7.0$ & $0.322$ & $0.107$ & $0.107$ & \nodata & \nodata & \nodata \\
SN\,2013gy & Si & $56641.4$ & $-7.0$ & $104.422$ & $4.290$ & $8.722$ & $10811$ & $45$ & $96$ \\
SN\,2013gy & C & $56643.4$ & $-5.0$ & $0.137$ & $0.046$ & $0.046$ & \nodata & \nodata & \nodata \\
SN\,2013gy & Si & $56643.4$ & $-5.0$ & $104.516$ & $3.141$ & $6.168$ & $10456$ & $35$ & $59$ \\
SN\,2013gy & C & $56646.5$ & $-2.0$ & $0.083$ & $0.028$ & $0.028$ & \nodata & \nodata & \nodata \\
SN\,2013gy & Si & $56646.5$ & $-2.0$ & $110.072$ & $3.010$ & $4.009$ & $10428$ & $54$ & $34$ \\
SN\,2013gy & C & $56647.7$ & $-0.8$ & $0.477$ & $0.159$ & $0.159$ & \nodata & \nodata & \nodata \\
SN\,2013gy & Si & $56647.7$ & $-0.8$ & $107.321$ & $3.100$ & $5.903$ & $9957$ & $90$ & $48$ \\
ASASSN-14lp & C & $57001.6$ & $-13.6$ & $5.120$ & $1.581$ & $1.308$ & $18457$ & $910$ & $707$ \\
ASASSN-14lp & Si & $57001.6$ & $-13.6$ & $78.969$ & $15.079$ & $16.059$ & $18035$ & $606$ & $625$ \\
ASASSN-14lp & HV Si & $57001.6$ & $-13.6$ & $21.075$ & $13.731$ & $11.724$ & $23508$ & $205$ & $540$ \\
ASASSN-14lp & C & $57003.5$ & $-11.7$ & $0.930$ & $0.922$ & $0.635$ & $16088$ & $552$ & $324$ \\
ASASSN-14lp & Si & $57003.5$ & $-11.7$ & $69.944$ & $7.338$ & $6.972$ & $16495$ & $537$ & $402$ \\
ASASSN-14lp & HV Si & $57003.5$ & $-11.7$ & $21.283$ & $7.656$ & $8.495$ & $20861$ & $524$ & $396$ \\
ASASSN-14lp & C & $57004.3$ & $-10.9$ & $0.447$ & $0.589$ & $0.217$ & $14446$ & $527$ & $422$ \\
ASASSN-14lp & Si & $57004.3$ & $-10.9$ & $63.759$ & $7.165$ & $13.658$ & $14114$ & $293$ & $689$ \\
ASASSN-14lp & HV Si & $57004.3$ & $-10.9$ & $21.003$ & $11.170$ & $4.342$ & $18972$ & $218$ & $344$ \\
ASASSN-14lp & C & $57005.5$ & $-9.8$ & $0.569$ & $0.394$ & $0.383$ & $15830$ & $335$ & $169$ \\
ASASSN-14lp & Si & $57005.5$ & $-9.8$ & $48.502$ & $5.248$ & $6.539$ & $14245$ & $214$ & $152$ \\
ASASSN-14lp & HV Si & $57005.5$ & $-9.8$ & $11.487$ & $2.819$ & $2.251$ & $19053$ & $209$ & $226$ \\
ASASSN-14lp & C & $57006.5$ & $-8.8$ & $0.504$ & $0.168$ & $0.168$ & \nodata & \nodata & \nodata \\
ASASSN-14lp & Si & $57006.5$ & $-8.8$ & $48.917$ & $4.256$ & $5.778$ & $13815$ & $107$ & $145$ \\
ASASSN-14lp & HV Si & $57006.5$ & $-8.8$ & $10.276$ & $3.145$ & $1.885$ & $19507$ & $205$ & $175$ \\
ASASSN-14lp & C & $57010.5$ & $-4.8$ & $0.263$ & $0.072$ & $0.072$ & \nodata & \nodata & \nodata \\
ASASSN-14lp & Si & $57010.5$ & $-4.8$ & $52.545$ & $6.935$ & $7.090$ & $12701$ & $107$ & $145$ \\
ASASSN-14lp & Si & $57011.5$ & $-3.8$ & $58.054$ & $4.372$ & $6.921$ & $12635$ & $66$ & $134$ \\
ASASSN-14lp & Si & $57012.5$ & $-2.8$ & $60.273$ & $3.552$ & $4.822$ & $12603$ & $40$ & $65$ \\
ASASSN-14lp & Si & $57014.3$ & $-1.0$ & $67.921$ & $2.680$ & $5.510$ & $10876$ & $32$ & $68$ \\
iPTF14bdn & C & $56807.7$ & $-14.6$ & $9.275$ & $2.993$ & $2.810$ & $19751$ & $1401$ & $1156$ \\
iPTF14bdn & Si & $56807.7$ & $-14.6$ & $6.039$ & $2.532$ & $1.599$ & $16698$ & $338$ & $444$ \\
iPTF14bdn & C & $56809.6$ & $-12.7$ & $6.398$ & $1.269$ & $1.119$ & $18401$ & $270$ & $284$ \\
iPTF14bdn & Si & $56809.6$ & $-12.7$ & $10.829$ & $2.169$ & $3.593$ & $15285$ & $257$ & $312$ \\
iPTF14bdn & C & $56811.7$ & $-10.6$ & $9.476$ & $1.653$ & $1.618$ & $18134$ & $278$ & $264$ \\
iPTF14bdn & Si & $56811.7$ & $-10.6$ & $12.441$ & $1.912$ & $2.817$ & $14762$ & $368$ & $393$ \\
iPTF14bdn & C & $56817.7$ & $-4.7$ & $1.300$ & $0.433$ & $0.433$ & \nodata & \nodata & \nodata \\
iPTF14bdn & Si & $56817.7$ & $-4.7$ & $25.104$ & $6.352$ & $4.553$ & $9639$ & $339$ & $233$ \\
SN\,2015bq & C & $57068.1$ & $-15.6$ & $1.749$ & $0.583$ & $0.583$ & \nodata & \nodata & \nodata \\
SN\,2015bq & Si & $57068.1$ & $-15.6$ & $11.700$ & $9.736$ & $6.868$ & $20131$ & $1834$ & $1890$ \\
SN\,2015bq & C & $57071.9$ & $-11.9$ & $2.183$ & $0.728$ & $0.728$ & \nodata & \nodata & \nodata \\
SN\,2015bq & Si & $57071.9$ & $-11.9$ & $24.074$ & $6.591$ & $5.608$ & $13999$ & $725$ & $851$ \\
SN\,2015bq & C & $57073.9$ & $-9.9$ & $1.726$ & $0.575$ & $0.575$ & \nodata & \nodata & \nodata \\
SN\,2015bq & Si & $57073.9$ & $-9.9$ & $24.877$ & $5.632$ & $4.593$ & $12759$ & $550$ & $513$ \\
SN\,2015bq & C & $57074.8$ & $-9.0$ & $2.603$ & $0.868$ & $0.868$ & \nodata & \nodata & \nodata \\
SN\,2015bq & Si & $57074.8$ & $-9.0$ & $32.540$ & $8.652$ & $8.053$ & $12515$ & $1160$ & $1028$ \\
SN\,2015bq & C & $57075.9$ & $-8.0$ & $1.221$ & $0.407$ & $0.407$ & \nodata & \nodata & \nodata \\
SN\,2015bq & Si & $57075.9$ & $-8.0$ & $29.450$ & $4.152$ & $3.964$ & $12481$ & $372$ & $348$ \\
SN\,2015bq & C & $57078.9$ & $-5.1$ & $1.423$ & $0.474$ & $0.474$ & \nodata & \nodata & \nodata \\
SN\,2015bq & Si & $57078.9$ & $-5.1$ & $36.674$ & $3.453$ & $3.501$ & $11122$ & $197$ & $188$ \\
SN\,2015bq & C & $57082.8$ & $-1.3$ & $1.180$ & $0.393$ & $0.393$ & \nodata & \nodata & \nodata \\
SN\,2015bq & Si & $57082.8$ & $-1.3$ & $44.715$ & $4.052$ & $5.439$ & $10092$ & $113$ & $120$ \\
SN\,2015F & C & $57092.0$ & $-14.4$ & $1.319$ & $0.440$ & $0.440$ & \nodata & \nodata & \nodata \\
SN\,2015F & Si & $57092.0$ & $-14.4$ & $133.407$ & $4.682$ & $4.865$ & $14667$ & $91$ & $92$ \\
SN\,2015F & C & $57094.2$ & $-12.2$ & $0.274$ & $0.091$ & $0.091$ & \nodata & \nodata & \nodata \\
SN\,2015F & Si & $57094.2$ & $-12.2$ & $110.136$ & $3.824$ & $4.314$ & $11838$ & $35$ & $31$ \\
SN\,2015F & Si & $57100.1$ & $-6.4$ & $92.431$ & $2.092$ & $5.754$ & $10630$ & $72$ & $34$ \\
SN\,2015F & C & $57100.1$ & $-6.4$ & $0.113$ & $0.304$ & $0.110$ & $10963$ & $356$ & $435$ \\
SN\,2015F & Si & $57102.0$ & $-4.5$ & $95.146$ & $2.161$ & $6.413$ & $10216$ & $81$ & $30$ \\
SN\,2015F & C & $57102.0$ & $-4.5$ & $0.081$ & $0.259$ & $0.081$ & $10623$ & $375$ & $870$ \\
SN\,2015F & C & $57103.7$ & $-2.8$ & $0.253$ & $0.084$ & $0.084$ & \nodata & \nodata & \nodata \\
SN\,2015F & Si & $57103.7$ & $-2.8$ & $88.694$ & $4.576$ & $9.861$ & $9870$ & $82$ & $63$ \\
iPTF16abc & C & $57484.2$ & $-14.3$ & $14.241$ & $2.071$ & $1.791$ & $13950$ & $249$ & $241$ \\
iPTF16abc & Si & $57484.2$ & $-14.3$ & $27.675$ & $4.030$ & $5.425$ & $13745$ & $214$ & $222$ \\
iPTF16abc & C & $57488.2$ & $-10.4$ & $2.478$ & $1.947$ & $1.718$ & $12140$ & $1350$ & $595$ \\
iPTF16abc & Si & $57488.2$ & $-10.4$ & $25.792$ & $3.882$ & $4.035$ & $10717$ & $282$ & $193$ \\
iPTF16abc & C & $57491.2$ & $-7.4$ & $0.526$ & $0.347$ & $0.247$ & $11251$ & $227$ & $207$ \\
iPTF16abc & Si & $57491.2$ & $-7.4$ & $28.406$ & $2.125$ & $5.585$ & $9918$ & $103$ & $142$ \\
iPTF16abc & C & $57494.1$ & $-4.6$ & $0.471$ & $0.882$ & $0.322$ & $10148$ & $553$ & $552$ \\
iPTF16abc & Si & $57494.1$ & $-4.6$ & $34.116$ & $2.527$ & $3.740$ & $10052$ & $74$ & $75$ \\
SN\,2017cbv & C & $57822.7$ & $-17.6$ & $41.814$ & $6.958$ & $7.233$ & $19323$ & $121$ & $116$ \\
SN\,2017cbv & HV Si & $57822.7$ & $-17.6$ & $45.161$ & $5.097$ & $5.433$ & $21878$ & $160$ & $154$ \\
SN\,2017cbv & C & $57824.8$ & $-15.5$ & $15.591$ & $3.674$ & $2.912$ & $15354$ & $410$ & $323$ \\
SN\,2017cbv & Si & $57824.8$ & $-15.5$ & $61.614$ & $3.621$ & $2.541$ & $16139$ & $122$ & $112$ \\
SN\,2017cbv & HV Si & $57824.8$ & $-15.5$ & $13.234$ & $0.951$ & $1.198$ & $21459$ & $78$ & $77$ \\
SN\,2017cbv & Si & $57828.6$ & $-11.8$ & $34.854$ & $8.408$ & $7.323$ & $10863$ & $325$ & $328$ \\
SN\,2017cbv & HV Si & $57828.6$ & $-11.8$ & $36.155$ & $7.866$ & $8.398$ & $16511$ & $453$ & $396$ \\
SN\,2017cbv & C & $57828.6$ & $-11.8$ & $0.388$ & $0.499$ & $0.360$ & $11101$ & $84$ & $269$ \\
SN\,2017cbv & Si & $57836.3$ & $-4.1$ & $53.809$ & $2.820$ & $5.494$ & $9894$ & $14$ & $50$ \\
SN\,2017cbv & HV Si & $57836.3$ & $-4.1$ & $4.358$ & $1.085$ & $2.545$ & $15955$ & $304$ & $838$ \\
SN\,2017cbv & C & $57836.3$ & $-4.1$ & $0.041$ & $0.122$ & $0.041$ & $10430$ & $342$ & $925$ \\
SN\,2017cbv & Si & $57837.1$ & $-3.3$ & $59.137$ & $2.860$ & $3.837$ & $10270$ & $72$ & $68$ \\
SN\,2017cbv & Si & $57838.3$ & $-2.1$ & $62.705$ & $2.850$ & $6.073$ & $10087$ & $90$ & $74$ \\
SN\,2017cbv & Si & $57839.7$ & $-0.7$ & $70.639$ & $3.193$ & $5.099$ & $9523$ & $62$ & $54$ \\
SN\,2017cfd & C & $57830.2$ & $-13.0$ & $0.668$ & $0.830$ & $0.537$ & $13214$ & $259$ & $165$ \\
SN\,2017cfd & Si & $57830.2$ & $-13.0$ & $56.772$ & $6.364$ & $11.035$ & $12470$ & $104$ & $200$ \\
SN\,2017cfd & HV Si & $57830.2$ & $-13.0$ & $14.935$ & $0.708$ & $1.212$ & $16467$ & $177$ & $401$ \\
SN\,2017cfd & C & $57843.3$ & $-0.1$ & $0.290$ & $0.097$ & $0.097$ & \nodata & \nodata & \nodata \\
SN\,2017cfd & Si & $57843.3$ & $-0.1$ & $98.508$ & $1.574$ & $3.744$ & $10661$ & $27$ & $26$ \\
SN\,2017cyy & C & $57859.0$ & $-11.0$ & $1.024$ & $2.154$ & $0.801$ & $12344$ & $362$ & $251$ \\
SN\,2017cyy & Si & $57859.0$ & $-11.0$ & $87.102$ & $4.638$ & $3.617$ & $12325$ & $61$ & $70$ \\
SN\,2017cyy & C & $57867.1$ & $-3.0$ & $0.060$ & $0.171$ & $0.060$ & $10868$ & $791$ & $558$ \\
SN\,2017cyy & Si & $57867.1$ & $-3.0$ & $85.519$ & $2.108$ & $6.000$ & $10739$ & $88$ & $23$ \\
SN\,2017erp & C & $57917.9$ & $-16.4$ & $13.706$ & $2.729$ & $2.462$ & $16264$ & $161$ & $172$ \\
SN\,2017erp & Si & $57917.9$ & $-16.4$ & $42.498$ & $21.797$ & $15.160$ & $16589$ & $1478$ & $915$ \\
SN\,2017erp & HV Si & $57917.9$ & $-16.4$ & $78.489$ & $17.447$ & $29.802$ & $22712$ & $737$ & $590$ \\
SN\,2017erp & C & $57918.8$ & $-15.5$ & $6.027$ & $0.888$ & $1.467$ & $14210$ & $58$ & $73$ \\
SN\,2017erp & Si & $57918.8$ & $-15.5$ & $101.143$ & $15.232$ & $7.263$ & $17061$ & $554$ & $185$ \\
SN\,2017erp & HV Si & $57918.8$ & $-15.5$ & $35.824$ & $1.914$ & $10.028$ & $22257$ & $102$ & $114$ \\
SN\,2017erp & C & $57919.7$ & $-14.6$ & $1.295$ & $0.211$ & $0.551$ & $13299$ & $139$ & $49$ \\
SN\,2017erp & Si & $57919.7$ & $-14.6$ & $104.005$ & $1.746$ & $4.039$ & $15855$ & $41$ & $70$ \\
SN\,2017erp & HV Si & $57919.7$ & $-14.6$ & $34.916$ & $0.865$ & $0.612$ & $20981$ & $26$ & $68$ \\
SN\,2017erp & Si & $57920.7$ & $-13.6$ & $93.782$ & $3.958$ & $3.894$ & $14708$ & $65$ & $115$ \\
SN\,2017erp & HV Si & $57920.7$ & $-13.6$ & $46.362$ & $3.619$ & $2.528$ & $19784$ & $46$ & $59$ \\
SN\,2017erp & C & $57920.7$ & $-13.6$ & $0.164$ & $0.436$ & $0.123$ & $13241$ & $254$ & $1434$ \\
SN\,2017erp & C & $57922.7$ & $-11.6$ & $0.082$ & $0.027$ & $0.027$ & \nodata & \nodata & \nodata \\
SN\,2017erp & Si & $57922.7$ & $-11.6$ & $83.477$ & $5.936$ & $13.899$ & $13203$ & $214$ & $422$ \\
SN\,2017erp & HV Si & $57922.7$ & $-11.6$ & $51.164$ & $11.688$ & $8.056$ & $18713$ & $130$ & $320$ \\
SN\,2017erp & C & $57924.2$ & $-10.1$ & $0.179$ & $0.060$ & $0.060$ & \nodata & \nodata & \nodata \\
SN\,2017erp & Si & $57924.2$ & $-10.1$ & $76.247$ & $3.311$ & $4.353$ & $12432$ & $199$ & $185$ \\
SN\,2017erp & HV Si & $57924.2$ & $-10.1$ & $43.425$ & $6.051$ & $8.184$ & $18235$ & $97$ & $142$ \\
SN\,2017erp & C & $57925.3$ & $-9.0$ & $0.213$ & $0.071$ & $0.071$ & \nodata & \nodata & \nodata \\
SN\,2017erp & Si & $57925.3$ & $-9.0$ & $78.583$ & $3.743$ & $6.388$ & $12173$ & $112$ & $172$ \\
SN\,2017erp & HV Si & $57925.3$ & $-9.0$ & $32.418$ & $4.929$ & $4.658$ & $18058$ & $123$ & $231$ \\
SN\,2017erp & C & $57927.2$ & $-7.2$ & $0.182$ & $0.061$ & $0.061$ & \nodata & \nodata & \nodata \\
SN\,2017erp & Si & $57927.2$ & $-7.2$ & $80.929$ & $4.956$ & $4.080$ & $11676$ & $42$ & $78$ \\
SN\,2017erp & HV Si & $57927.2$ & $-7.2$ & $16.729$ & $4.000$ & $5.637$ & $17693$ & $275$ & $270$ \\
SN\,2017erp & C & $57928.2$ & $-6.2$ & $0.116$ & $0.039$ & $0.039$ & \nodata & \nodata & \nodata \\
SN\,2017erp & Si & $57928.2$ & $-6.2$ & $81.749$ & $3.278$ & $4.704$ & $11460$ & $20$ & $45$ \\
SN\,2017erp & HV Si & $57928.2$ & $-6.2$ & $9.038$ & $5.352$ & $2.970$ & $17317$ & $221$ & $340$ \\
SN\,2017erp & C & $57929.2$ & $-5.2$ & $1.670$ & $0.557$ & $0.557$ & \nodata & \nodata & \nodata \\
SN\,2017erp & Si & $57929.2$ & $-5.2$ & $71.768$ & $5.054$ & $5.814$ & $11229$ & $100$ & $109$ \\
SN\,2017erp & HV Si & $57929.2$ & $-5.2$ & $2.588$ & $1.979$ & $1.183$ & $16460$ & $298$ & $269$ \\
SN\,2017erp & C & $57930.2$ & $-4.2$ & $0.137$ & $0.046$ & $0.046$ & \nodata & \nodata & \nodata \\
SN\,2017erp & Si & $57930.2$ & $-4.2$ & $88.577$ & $2.857$ & $6.233$ & $11034$ & $30$ & $41$ \\
SN\,2017erp & HV Si & $57930.2$ & $-4.2$ & $3.800$ & $1.013$ & $2.062$ & $17341$ & $168$ & $388$ \\
SN\,2017erp & C & $57931.3$ & $-3.1$ & $0.138$ & $0.046$ & $0.046$ & \nodata & \nodata & \nodata \\
SN\,2017erp & Si & $57931.3$ & $-3.1$ & $90.275$ & $2.019$ & $4.123$ & $10965$ & $35$ & $23$ \\
SN\,2017erp & HV Si & $57931.3$ & $-3.1$ & $2.522$ & $0.634$ & $0.926$ & $17273$ & $153$ & $234$ \\
SN\,2017erp & C & $57933.2$ & $-1.2$ & $0.119$ & $0.040$ & $0.040$ & \nodata & \nodata & \nodata \\
SN\,2017erp & Si & $57933.2$ & $-1.2$ & $93.720$ & $2.773$ & $5.010$ & $10556$ & $59$ & $29$ \\
SN\,2017erp & HV Si & $57933.2$ & $-1.2$ & $1.144$ & $0.825$ & $0.561$ & $16997$ & $235$ & $206$ \\
SN\,2017fgc & C & $57945.5$ & $-13.9$ & $0.840$ & $0.280$ & $0.280$ & \nodata & \nodata & \nodata \\
SN\,2017fgc & Si & $57945.5$ & $-13.9$ & $166.217$ & $5.757$ & $5.635$ & $20055$ & $66$ & $73$ \\
SN\,2017fgc & C & $57952.5$ & $-6.9$ & $0.293$ & $0.098$ & $0.098$ & \nodata & \nodata & \nodata \\
SN\,2017fgc & Si & $57952.5$ & $-6.9$ & $148.018$ & $2.611$ & $13.381$ & $16398$ & $43$ & $145$ \\
SN\,2017fgc & Si & $57960.5$ & $1.0$ & $152.125$ & $2.880$ & $4.378$ & $14919$ & $41$ & $47$ \\
ASASSN-18bt & C & $58155.2$ & $-7.4$ & $2.602$ & $1.089$ & $1.858$ & $11505$ & $93$ & $82$ \\
ASASSN-18bt & Si & $58155.2$ & $-7.4$ & $60.854$ & $3.735$ & $4.906$ & $10778$ & $59$ & $65$ \\
ASASSN-18bt & C & $58155.7$ & $-6.9$ & $3.550$ & $0.873$ & $0.907$ & $11443$ & $104$ & $105$ \\
ASASSN-18bt & Si & $58155.7$ & $-6.9$ & $64.491$ & $4.149$ & $4.804$ & $10671$ & $57$ & $61$ \\
ASASSN-18bt & C & $58156.3$ & $-6.3$ & $3.453$ & $0.832$ & $0.636$ & $11342$ & $78$ & $81$ \\
ASASSN-18bt & Si & $58156.3$ & $-6.3$ & $66.830$ & $3.034$ & $4.463$ & $10606$ & $35$ & $45$ \\
ASASSN-18bt & C & $58158.4$ & $-4.3$ & $2.265$ & $0.391$ & $0.468$ & $10570$ & $67$ & $68$ \\
ASASSN-18bt & Si & $58158.4$ & $-4.3$ & $66.797$ & $0.867$ & $1.746$ & $10282$ & $14$ & $16$ \\
ASASSN-18bt & Si & $58163.2$ & $0.5$ & $79.581$ & $2.242$ & $3.591$ & $9809$ & $53$ & $33$ \\
SN\,2018agk & C & $58192.9$ & $-11.0$ & $1.318$ & $1.478$ & $0.916$ & $10667$ & $64$ & $170$ \\
SN\,2018agk & Si & $58192.9$ & $-11.0$ & $67.624$ & $6.960$ & $4.506$ & $11655$ & $119$ & $95$ \\
SN\,2018agk & Si & $58194.1$ & $-9.8$ & $56.932$ & $9.679$ & $23.133$ & $10307$ & $366$ & $580$ \\
SN\,2018agk & HV Si & $58194.1$ & $-9.8$ & $25.341$ & $15.417$ & $9.832$ & $14532$ & $348$ & $949$ \\
SN\,2018agk & C & $58194.1$ & $-9.8$ & $0.616$ & $1.030$ & $0.495$ & $11068$ & $396$ & $580$ \\
SN\,2018agk & C & $58196.3$ & $-7.7$ & $0.708$ & $0.236$ & $0.236$ & \nodata & \nodata & \nodata \\
SN\,2018agk & Si & $58196.3$ & $-7.7$ & $59.449$ & $5.278$ & $7.603$ & $10558$ & $79$ & $137$ \\
SN\,2018agk & HV Si & $58196.3$ & $-7.7$ & $5.497$ & $4.191$ & $2.196$ & $14940$ & $318$ & $627$ \\
SN\,2018agk & C & $58199.6$ & $-4.5$ & $0.018$ & $0.006$ & $0.006$ & \nodata & \nodata & \nodata \\
SN\,2018agk & Si & $58199.6$ & $-4.5$ & $69.407$ & $4.693$ & $60.950$ & $10151$ & $39$ & $3158$ \\
SN\,2018agk & HV Si & $58199.6$ & $-4.5$ & $2.549$ & $53.155$ & $0.934$ & $14783$ & $621$ & $4332$ \\
SN\,2018agk & C & $58200.9$ & $-3.2$ & $0.614$ & $0.205$ & $0.205$ & \nodata & \nodata & \nodata \\
SN\,2018agk & Si & $58200.9$ & $-3.2$ & $77.509$ & $3.330$ & $8.096$ & $10308$ & $49$ & $96$ \\
SN\,2018agk & C & $58201.3$ & $-2.8$ & $0.940$ & $0.313$ & $0.313$ & \nodata & \nodata & \nodata \\
SN\,2018agk & Si & $58201.3$ & $-2.8$ & $78.253$ & $3.897$ & $6.131$ & $10033$ & $64$ & $90$ \\
SN\,2018aoz & C & $58210.4$ & $-11.7$ & $0.702$ & $0.234$ & $0.234$ & \nodata & \nodata & \nodata \\
SN\,2018aoz & Si & $58210.4$ & $-11.7$ & $66.693$ & $3.632$ & $7.662$ & $11211$ & $389$ & $363$ \\
SN\,2018aoz & HV Si & $58210.4$ & $-11.7$ & $45.983$ & $5.959$ & $6.183$ & $15600$ & $211$ & $189$ \\
SN\,2018aoz & C & $58213.7$ & $-8.5$ & $0.273$ & $0.091$ & $0.091$ & \nodata & \nodata & \nodata \\
SN\,2018aoz & Si & $58213.7$ & $-8.5$ & $67.095$ & $6.024$ & $10.500$ & $10766$ & $193$ & $183$ \\
SN\,2018aoz & HV Si & $58213.7$ & $-8.5$ & $27.062$ & $5.685$ & $2.798$ & $14134$ & $75$ & $94$ \\
SN\,2018aoz & C & $58214.3$ & $-7.9$ & $0.421$ & $0.140$ & $0.140$ & \nodata & \nodata & \nodata \\
SN\,2018aoz & Si & $58214.3$ & $-7.9$ & $97.509$ & $3.238$ & $3.131$ & $12008$ & $38$ & $38$ \\
SN\,2018aoz & C & $58216.6$ & $-5.6$ & $0.150$ & $0.050$ & $0.050$ & \nodata & \nodata & \nodata \\
SN\,2018aoz & Si & $58216.6$ & $-5.6$ & $103.772$ & $1.806$ & $2.461$ & $11355$ & $28$ & $27$ \\
SN\,2018aoz & C & $58219.5$ & $-2.7$ & $0.132$ & $0.044$ & $0.044$ & \nodata & \nodata & \nodata \\
SN\,2018aoz & Si & $58219.5$ & $-2.7$ & $107.170$ & $1.666$ & $3.391$ & $11178$ & $21$ & $28$ \\
SN\,2018gv & C & $58134.4$ & $-15.2$ & $8.950$ & $0.842$ & $0.681$ & $14980$ & $49$ & $49$ \\
SN\,2018gv & Si & $58134.4$ & $-15.2$ & $122.338$ & $1.540$ & $7.019$ & $16320$ & $20$ & $58$ \\
SN\,2018gv & C & $58135.3$ & $-14.3$ & $5.523$ & $1.031$ & $1.852$ & $14800$ & $35$ & $25$ \\
SN\,2018gv & Si & $58135.3$ & $-14.3$ & $122.410$ & $1.189$ & $3.098$ & $15087$ & $40$ & $15$ \\
SN\,2018gv & C & $58136.5$ & $-13.1$ & $3.375$ & $1.006$ & $1.195$ & $14198$ & $73$ & $66$ \\
SN\,2018gv & Si & $58136.5$ & $-13.1$ & $111.461$ & $2.488$ & $3.313$ & $14215$ & $32$ & $32$ \\
SN\,2018gv & C & $58138.4$ & $-11.2$ & $1.120$ & $0.786$ & $0.708$ & $13453$ & $113$ & $38$ \\
SN\,2018gv & Si & $58138.4$ & $-11.2$ & $89.306$ & $2.020$ & $2.763$ & $12863$ & $29$ & $21$ \\
SN\,2018gv & C & $58141.4$ & $-8.3$ & $0.073$ & $0.024$ & $0.024$ & \nodata & \nodata & \nodata \\
SN\,2018gv & Si & $58141.4$ & $-8.3$ & $77.023$ & $1.292$ & $1.566$ & $11842$ & $19$ & $20$ \\
SN\,2018gv & C & $58143.3$ & $-6.4$ & $0.320$ & $0.107$ & $0.107$ & \nodata & \nodata & \nodata \\
SN\,2018gv & Si & $58143.3$ & $-6.4$ & $78.389$ & $1.593$ & $2.861$ & $11505$ & $25$ & $30$ \\
SN\,2018gv & C & $58147.3$ & $-2.4$ & $0.048$ & $0.016$ & $0.016$ & \nodata & \nodata & \nodata \\
SN\,2018gv & Si & $58147.3$ & $-2.4$ & $82.405$ & $1.132$ & $3.085$ & $10922$ & $28$ & $13$ \\
SN\,2018xx & C & $58171.2$ & $-12.6$ & $1.530$ & $0.719$ & $1.326$ & $14176$ & $347$ & $336$ \\
SN\,2018xx & Si & $58171.2$ & $-12.6$ & $162.286$ & $3.826$ & $7.170$ & $15988$ & $32$ & $47$ \\
SN\,2018yu & C & $58178.5$ & $-15.7$ & $17.357$ & $4.203$ & $3.611$ & $13687$ & $324$ & $285$ \\
SN\,2018yu & Si & $58178.5$ & $-15.7$ & $105.464$ & $6.283$ & $7.728$ & $14773$ & $201$ & $227$ \\
SN\,2018yu & HV Si & $58178.5$ & $-15.7$ & $16.461$ & $4.277$ & $3.555$ & $20959$ & $356$ & $440$ \\
SN\,2018yu & C & $58187.0$ & $-7.2$ & $0.198$ & $0.476$ & $0.167$ & $9916$ & $401$ & $398$ \\
SN\,2018yu & Si & $58187.0$ & $-7.2$ & $73.433$ & $3.594$ & $6.416$ & $10171$ & $124$ & $63$ \\
SN\,2019ein & C & $58605.3$ & $-14.1$ & $11.112$ & $1.352$ & $3.212$ & $18907$ & $117$ & $71$ \\
SN\,2019ein & Si & $58605.3$ & $-14.1$ & $127.850$ & $2.919$ & $5.805$ & $21329$ & $55$ & $56$ \\
SN\,2019ein & HV Si & $58605.3$ & $-14.1$ & $35.435$ & $1.162$ & $1.155$ & $26169$ & $29$ & $51$ \\
SN\,2019ein & C & $58606.8$ & $-12.6$ & $1.186$ & $0.395$ & $0.395$ & \nodata & \nodata & \nodata \\
SN\,2019ein & Si & $58606.8$ & $-12.6$ & $116.001$ & $10.002$ & $11.549$ & $18907$ & $290$ & $354$ \\
SN\,2019ein & HV Si & $58606.8$ & $-12.6$ & $48.274$ & $10.433$ & $8.889$ & $24088$ & $162$ & $213$ \\
SN\,2019ein & C & $58607.0$ & $-12.4$ & $2.744$ & $0.915$ & $0.915$ & \nodata & \nodata & \nodata \\
SN\,2019ein & Si & $58607.0$ & $-12.4$ & $86.030$ & $12.469$ & $13.273$ & $18687$ & $267$ & $333$ \\
SN\,2019ein & HV Si & $58607.0$ & $-12.4$ & $29.979$ & $9.144$ & $6.476$ & $23392$ & $292$ & $357$ \\
SN\,2019ein & C & $58608.0$ & $-11.4$ & $0.917$ & $0.891$ & $0.811$ & $15000$ & $679$ & $318$ \\
SN\,2019ein & Si & $58608.0$ & $-11.4$ & $91.913$ & $31.565$ & $30.131$ & $16578$ & $973$ & $1028$ \\
SN\,2019ein & HV Si & $58608.0$ & $-11.4$ & $70.400$ & $28.595$ & $28.576$ & $21942$ & $622$ & $808$ \\
SN\,2019ein & C & $58609.5$ & $-9.9$ & $0.159$ & $0.053$ & $0.053$ & \nodata & \nodata & \nodata \\
SN\,2019ein & Si & $58609.5$ & $-9.9$ & $147.484$ & $4.565$ & $14.189$ & $17946$ & $95$ & $123$ \\
SN\,2019ein & C & $58610.7$ & $-8.7$ & $0.272$ & $0.091$ & $0.091$ & \nodata & \nodata & \nodata \\
SN\,2019ein & Si & $58610.7$ & $-8.7$ & $134.611$ & $3.755$ & $8.256$ & $16936$ & $133$ & $59$ \\
SN\,2019ein & Si & $58611.5$ & $-7.9$ & $135.275$ & $3.441$ & $7.324$ & $16316$ & $53$ & $97$ \\
SN\,2019ein & C & $58611.5$ & $-7.9$ & $0.107$ & $0.194$ & $0.070$ & $14273$ & $41$ & $30$ \\
SN\,2019ein & C & $58613.8$ & $-5.7$ & $0.096$ & $0.169$ & $0.079$ & $13510$ & $107$ & $49$ \\
SN\,2019ein & Si & $58613.8$ & $-5.7$ & $121.326$ & $2.190$ & $4.775$ & $14307$ & $40$ & $41$ \\
SN\,2019ein & C & $58615.3$ & $-4.2$ & $0.084$ & $0.115$ & $0.058$ & $13606$ & $48$ & $72$ \\
SN\,2019ein & Si & $58615.3$ & $-4.2$ & $121.409$ & $2.246$ & $6.157$ & $15014$ & $32$ & $76$ \\
SN\,2019ein & C & $58616.5$ & $-3.0$ & $0.386$ & $0.395$ & $0.242$ & $13462$ & $179$ & $103$ \\
SN\,2019ein & Si & $58616.5$ & $-3.0$ & $119.186$ & $3.048$ & $6.060$ & $13747$ & $44$ & $53$ \\
SN\,2019ein & C & $58617.8$ & $-1.7$ & $0.208$ & $0.069$ & $0.069$ & \nodata & \nodata & \nodata \\
SN\,2019ein & Si & $58617.8$ & $-1.7$ & $122.855$ & $3.364$ & $6.545$ & $12831$ & $33$ & $61$ \\
SN\,2019ein & C & $58619.2$ & $-0.3$ & $0.455$ & $0.152$ & $0.152$ & \nodata & \nodata & \nodata \\
SN\,2019ein & Si & $58619.2$ & $-0.3$ & $116.936$ & $2.592$ & $4.548$ & $13633$ & $33$ & $38$ \\
SN\,2019np & C & $58493.5$ & $-16.6$ & $31.150$ & $2.481$ & $8.713$ & $14901$ & $177$ & $76$ \\
SN\,2019np & Si & $58493.5$ & $-16.6$ & $99.752$ & $3.264$ & $6.216$ & $14362$ & $66$ & $84$ \\
SN\,2019np & HV Si & $58493.5$ & $-16.6$ & $25.783$ & $1.302$ & $1.064$ & $19367$ & $92$ & $153$ \\
SN\,2019np & C & $58493.6$ & $-16.5$ & $30.492$ & $1.960$ & $1.811$ & $14890$ & $351$ & $63$ \\
SN\,2019np & Si & $58493.6$ & $-16.5$ & $131.216$ & $1.523$ & $12.109$ & $15576$ & $29$ & $41$ \\
SN\,2019np & C & $58495.7$ & $-14.4$ & $4.531$ & $1.949$ & $1.786$ & $13128$ & $157$ & $141$ \\
SN\,2019np & Si & $58495.7$ & $-14.4$ & $114.303$ & $3.082$ & $3.209$ & $13435$ & $44$ & $42$ \\
SN\,2019np & C & $58496.1$ & $-14.0$ & $5.424$ & $1.362$ & $3.470$ & $12857$ & $243$ & $183$ \\
SN\,2019np & Si & $58496.1$ & $-14.0$ & $102.067$ & $3.260$ & $3.946$ & $13187$ & $38$ & $34$ \\
SN\,2019np & C & $58497.1$ & $-13.0$ & $2.703$ & $0.966$ & $2.066$ & $12228$ & $95$ & $129$ \\
SN\,2019np & Si & $58497.1$ & $-13.0$ & $85.356$ & $4.034$ & $10.853$ & $12569$ & $51$ & $93$ \\
SN\,2019np & C & $58498.2$ & $-11.9$ & $3.332$ & $0.888$ & $2.377$ & $12062$ & $72$ & $73$ \\
SN\,2019np & Si & $58498.2$ & $-11.9$ & $79.697$ & $3.568$ & $5.164$ & $11994$ & $40$ & $59$ \\
SN\,2019np & C & $58499.7$ & $-10.5$ & $2.151$ & $0.841$ & $1.110$ & $11669$ & $79$ & $78$ \\
SN\,2019np & Si & $58499.7$ & $-10.5$ & $75.736$ & $2.953$ & $9.130$ & $11425$ & $40$ & $83$ \\
SN\,2019np & C & $58503.2$ & $-7.0$ & $1.386$ & $0.832$ & $0.542$ & $11059$ & $70$ & $69$ \\
SN\,2019np & Si & $58503.2$ & $-7.0$ & $65.106$ & $2.217$ & $5.669$ & $10704$ & $25$ & $31$ \\
SN\,2019np & Si & $58506.2$ & $-4.0$ & $71.321$ & $2.560$ & $4.806$ & $10251$ & $51$ & $40$ \\
SN\,2019np & C & $58506.2$ & $-4.0$ & $0.212$ & $0.758$ & $0.195$ & $10406$ & $418$ & $467$ \\
SN\,2019np & Si & $58506.9$ & $-3.3$ & $78.321$ & $2.351$ & $5.186$ & $10077$ & $86$ & $42$ \\
SN\,2019np & C & $58506.9$ & $-3.3$ & $0.183$ & $0.641$ & $0.152$ & $9998$ & $782$ & $237$ \\
SN\,2019np & C & $58507.8$ & $-2.4$ & $1.272$ & $0.424$ & $0.424$ & \nodata & \nodata & \nodata \\
SN\,2019np & Si & $58507.8$ & $-2.4$ & $78.827$ & $4.164$ & $6.981$ & $10134$ & $79$ & $80$ \\
SN\,2019np & Si & $58509.2$ & $-1.0$ & $78.870$ & $3.573$ & $5.816$ & $10011$ & $56$ & $43$ \\
SN\,2019np & C & $58509.2$ & $-1.0$ & $0.105$ & $0.373$ & $0.101$ & $9648$ & $1098$ & $210$ \\
SN\,2020nlb & C & $59025.8$ & $-16.0$ & $1.668$ & $0.556$ & $0.556$ & \nodata & \nodata & \nodata \\
SN\,2020nlb & Si & $59025.8$ & $-16.0$ & $135.391$ & $8.253$ & $7.827$ & $14028$ & $146$ & $149$ \\
SN\,2020nlb & C & $59029.0$ & $-12.8$ & $0.168$ & $0.056$ & $0.056$ & \nodata & \nodata & \nodata \\
SN\,2020nlb & Si & $59029.0$ & $-12.8$ & $97.412$ & $3.360$ & $4.969$ & $12136$ & $52$ & $44$ \\
SN\,2020nlb & C & $59036.0$ & $-5.8$ & $0.254$ & $0.085$ & $0.085$ & \nodata & \nodata & \nodata \\
SN\,2020nlb & Si & $59036.0$ & $-5.8$ & $105.592$ & $1.495$ & $5.764$ & $10965$ & $17$ & $35$ \\
SN\,2021aefx & C & $59529.9$ & $-16.5$ & $25.956$ & $1.589$ & $4.504$ & $21383$ & $82$ & $70$ \\
SN\,2021aefx & Si & $59529.9$ & $-16.5$ & $137.054$ & $4.575$ & $4.978$ & $24213$ & $162$ & $163$ \\
SN\,2021aefx & HV Si & $59529.9$ & $-16.5$ & $56.392$ & $1.867$ & $2.195$ & $30851$ & $164$ & $177$ \\
SN\,2021aefx & C & $59530.9$ & $-15.5$ & $5.951$ & $0.686$ & $1.751$ & $15030$ & $334$ & $146$ \\
SN\,2021aefx & Si & $59530.9$ & $-15.5$ & $116.880$ & $4.082$ & $3.986$ & $17932$ & $146$ & $156$ \\
SN\,2021aefx & HV Si & $59530.9$ & $-15.5$ & $98.794$ & $4.088$ & $3.851$ & $25441$ & $85$ & $89$ \\
SN\,2021aefx & C & $59532.8$ & $-13.6$ & $0.064$ & $0.021$ & $0.021$ & \nodata & \nodata & \nodata \\
SN\,2021aefx & Si & $59532.8$ & $-13.6$ & $120.211$ & $4.169$ & $11.134$ & $16161$ & $36$ & $174$ \\
SN\,2021aefx & HV Si & $59532.8$ & $-13.6$ & $30.977$ & $1.781$ & $1.037$ & $21502$ & $22$ & $302$ \\
SN\,2021aefx & C & $59533.6$ & $-12.8$ & $0.146$ & $0.049$ & $0.049$ & \nodata & \nodata & \nodata \\
SN\,2021aefx & Si & $59533.6$ & $-12.8$ & $117.505$ & $2.414$ & $10.336$ & $15776$ & $33$ & $95$ \\
SN\,2021aefx & HV Si & $59533.6$ & $-12.8$ & $23.924$ & $1.044$ & $1.020$ & $21068$ & $46$ & $261$ \\
SN\,2021aefx & C & $59534.5$ & $-11.9$ & $0.170$ & $0.057$ & $0.057$ & \nodata & \nodata & \nodata \\
SN\,2021aefx & Si & $59534.5$ & $-11.9$ & $115.762$ & $4.600$ & $5.902$ & $15079$ & $59$ & $71$ \\
SN\,2021aefx & HV Si & $59534.5$ & $-11.9$ & $20.419$ & $2.133$ & $0.772$ & $20774$ & $129$ & $190$ \\
SN\,2021aefx & C & $59535.1$ & $-11.3$ & $0.039$ & $0.013$ & $0.013$ & \nodata & \nodata & \nodata \\
SN\,2021aefx & Si & $59535.1$ & $-11.3$ & $110.346$ & $4.018$ & $8.641$ & $14831$ & $53$ & $157$ \\
SN\,2021aefx & HV Si & $59535.1$ & $-11.3$ & $15.764$ & $0.508$ & $0.296$ & $20590$ & $162$ & $389$ \\
SN\,2021aefx & C & $59536.9$ & $-9.6$ & $0.037$ & $0.012$ & $0.012$ & \nodata & \nodata & \nodata \\
SN\,2021aefx & Si & $59536.9$ & $-9.6$ & $99.309$ & $3.573$ & $10.464$ & $13876$ & $9$ & $52$ \\
SN\,2021aefx & HV Si & $59536.9$ & $-9.6$ & $8.592$ & $2.997$ & $3.370$ & $20355$ & $231$ & $580$ \\
SN\,2021aefx & C & $59538.1$ & $-8.4$ & $0.027$ & $0.009$ & $0.009$ & \nodata & \nodata & \nodata \\
SN\,2021aefx & Si & $59538.1$ & $-8.4$ & $96.277$ & $2.995$ & $7.093$ & $13418$ & $24$ & $31$ \\
SN\,2021aefx & HV Si & $59538.1$ & $-8.4$ & $3.992$ & $1.651$ & $1.272$ & $20101$ & $338$ & $509$ \\
SN\,2021aefx & C & $59538.9$ & $-7.6$ & $0.053$ & $0.018$ & $0.018$ & \nodata & \nodata & \nodata \\
SN\,2021aefx & Si & $59538.9$ & $-7.6$ & $96.203$ & $2.465$ & $5.513$ & $13138$ & $34$ & $24$ \\
SN\,2021aefx & HV Si & $59538.9$ & $-7.6$ & $2.235$ & $1.271$ & $0.855$ & $19931$ & $363$ & $354$ \\
SN\,2021aefx & Si & $59546.1$ & $-0.4$ & $97.457$ & $1.713$ & $6.411$ & $11659$ & $24$ & $70$ \\
SN\,2021fxy & C & $59291.1$ & $-13.9$ & $2.854$ & $0.581$ & $1.101$ & $12841$ & $172$ & $89$ \\
SN\,2021fxy & Si & $59291.1$ & $-13.9$ & $148.954$ & $7.903$ & $18.378$ & $16723$ & $200$ & $526$ \\
SN\,2021fxy & HV Si & $59291.1$ & $-13.9$ & $24.754$ & $16.131$ & $5.655$ & $22398$ & $108$ & $313$ \\
SN\,2021fxy & Si & $59299.1$ & $-5.9$ & $47.378$ & $9.788$ & $8.234$ & $10337$ & $247$ & $120$ \\
SN\,2021fxy & C & $59299.1$ & $-5.9$ & $0.056$ & $0.256$ & $0.048$ & $10674$ & $490$ & $111$ \\
SN\,2021fxy & Si & $59305.0$ & $-0.1$ & $77.794$ & $1.712$ & $4.342$ & $9721$ & $18$ & $16$ \\
SN\,2021hpr & C & $59307.0$ & $-14.3$ & $0.497$ & $0.166$ & $0.166$ & \nodata & \nodata & \nodata \\
SN\,2021hpr & Si & $59307.0$ & $-14.3$ & $192.997$ & $3.435$ & $3.783$ & $20438$ & $45$ & $45$ \\
SN\,2021hpr & C & $59308.0$ & $-13.3$ & $2.978$ & $0.993$ & $0.993$ & \nodata & \nodata & \nodata \\
SN\,2021hpr & Si & $59308.0$ & $-13.3$ & $194.330$ & $10.580$ & $10.304$ & $18915$ & $149$ & $152$ \\
SN\,2021hpr & C & $59309.3$ & $-12.0$ & $0.554$ & $0.185$ & $0.185$ & \nodata & \nodata & \nodata \\
SN\,2021hpr & Si & $59309.3$ & $-12.0$ & $162.336$ & $3.588$ & $3.817$ & $17646$ & $41$ & $42$ \\
SN\,2021hpr & C & $59310.0$ & $-11.3$ & $1.336$ & $0.445$ & $0.445$ & \nodata & \nodata & \nodata \\
SN\,2021hpr & Si & $59310.0$ & $-11.3$ & $154.790$ & $7.350$ & $8.261$ & $17543$ & $101$ & $98$ \\
SN\,2021hpr & C & $59311.0$ & $-10.3$ & $1.828$ & $0.609$ & $0.609$ & \nodata & \nodata & \nodata \\
SN\,2021hpr & Si & $59311.0$ & $-10.3$ & $149.454$ & $8.142$ & $8.265$ & $16513$ & $135$ & $131$ \\
SN\,2021hpr & C & $59313.0$ & $-8.3$ & $0.924$ & $0.308$ & $0.308$ & \nodata & \nodata & \nodata \\
SN\,2021hpr & Si & $59313.0$ & $-8.3$ & $122.789$ & $5.079$ & $7.523$ & $14834$ & $91$ & $111$ \\
SN\,2021hpr & C & $59314.4$ & $-6.9$ & $0.953$ & $0.318$ & $0.318$ & \nodata & \nodata & \nodata \\
SN\,2021hpr & Si & $59314.4$ & $-6.9$ & $80.444$ & $10.450$ & $41.950$ & $12790$ & $296$ & $1551$ \\
SN\,2021hpr & C & $59317.2$ & $-4.2$ & $0.310$ & $0.103$ & $0.103$ & \nodata & \nodata & \nodata \\
SN\,2021hpr & Si & $59317.2$ & $-4.2$ & $96.106$ & $3.384$ & $7.287$ & $12500$ & $70$ & $101$ \\
SN\,2021hpr & C & $59318.2$ & $-3.2$ & $0.259$ & $0.086$ & $0.086$ & \nodata & \nodata & \nodata \\
SN\,2021hpr & Si & $59318.2$ & $-3.2$ & $84.119$ & $3.743$ & $8.084$ & $11913$ & $36$ & $88$ \\
SN\,2021hpr & C & $59320.2$ & $-1.2$ & $0.224$ & $0.075$ & $0.075$ & \nodata & \nodata & \nodata \\
SN\,2021hpr & Si & $59320.2$ & $-1.2$ & $90.915$ & $2.908$ & $46.416$ & $11497$ & $1125$ & $21$ \\
SN\,2023bee & C & $59976.9$ & $-15.3$ & $28.093$ & $1.855$ & $3.892$ & $20049$ & $169$ & $121$ \\
SN\,2023bee & Si & $59976.9$ & $-15.3$ & $93.645$ & $2.861$ & $5.353$ & $22575$ & $90$ & $96$ \\
SN\,2023bee & HV Si & $59976.9$ & $-15.3$ & $14.976$ & $1.046$ & $1.176$ & $28833$ & $92$ & $138$ \\
SN\,2023bee & C & $59977.6$ & $-14.6$ & $14.867$ & $6.315$ & $5.340$ & $17191$ & $214$ & $216$ \\
SN\,2023bee & Si & $59977.6$ & $-14.6$ & $73.867$ & $10.527$ & $8.996$ & $19086$ & $378$ & $670$ \\
SN\,2023bee & HV Si & $59977.6$ & $-14.6$ & $43.887$ & $16.321$ & $8.393$ & $25047$ & $255$ & $253$ \\
SN\,2023bee & C & $59978.1$ & $-14.1$ & $13.090$ & $1.249$ & $0.912$ & $15498$ & $54$ & $57$ \\
SN\,2023bee & Si & $59978.1$ & $-14.1$ & $110.589$ & $2.147$ & $7.541$ & $18505$ & $100$ & $160$ \\
SN\,2023bee & HV Si & $59978.1$ & $-14.1$ & $41.054$ & $1.775$ & $1.586$ & $24424$ & $45$ & $109$ \\
SN\,2023bee & C & $59979.5$ & $-12.7$ & $1.561$ & $0.970$ & $0.900$ & $15270$ & $165$ & $163$ \\
SN\,2023bee & Si & $59979.5$ & $-12.7$ & $86.040$ & $2.598$ & $6.380$ & $17132$ & $108$ & $111$ \\
SN\,2023bee & HV Si & $59979.5$ & $-12.7$ & $33.521$ & $1.838$ & $1.872$ & $22477$ & $107$ & $140$ \\
SN\,2023bee & C & $59980.7$ & $-11.5$ & $0.480$ & $0.160$ & $0.160$ & \nodata & \nodata & \nodata \\
SN\,2023bee & Si & $59980.7$ & $-11.5$ & $69.510$ & $5.327$ & $10.480$ & $15490$ & $135$ & $259$ \\
SN\,2023bee & HV Si & $59980.7$ & $-11.5$ & $28.810$ & $1.796$ & $1.829$ & $21416$ & $135$ & $431$ \\
SN\,2023bee & C & $59981.7$ & $-10.5$ & $0.386$ & $0.129$ & $0.129$ & \nodata & \nodata & \nodata \\
SN\,2023bee & Si & $59981.7$ & $-10.5$ & $63.658$ & $7.562$ & $9.941$ & $14577$ & $122$ & $204$ \\
SN\,2023bee & HV Si & $59981.7$ & $-10.5$ & $23.055$ & $2.993$ & $2.981$ & $21226$ & $109$ & $530$ \\
SN\,2023bee & C & $59983.5$ & $-8.7$ & $0.215$ & $0.072$ & $0.072$ & \nodata & \nodata & \nodata \\
SN\,2023bee & Si & $59983.5$ & $-8.7$ & $56.518$ & $5.118$ & $7.841$ & $13091$ & $88$ & $148$ \\
SN\,2023bee & HV Si & $59983.5$ & $-8.7$ & $14.605$ & $2.910$ & $5.530$ & $20446$ & $330$ & $581$ \\
SN\,2023bee & C & $59984.6$ & $-7.6$ & $0.284$ & $0.095$ & $0.095$ & \nodata & \nodata & \nodata \\
SN\,2023bee & Si & $59984.6$ & $-7.6$ & $57.028$ & $5.149$ & $5.102$ & $12707$ & $37$ & $80$ \\
SN\,2023bee & HV Si & $59984.6$ & $-7.6$ & $7.711$ & $1.735$ & $2.901$ & $20416$ & $304$ & $724$ \\
SN\,2023bee & C & $59985.6$ & $-6.7$ & $0.204$ & $0.068$ & $0.068$ & \nodata & \nodata & \nodata \\
SN\,2023bee & Si & $59985.6$ & $-6.7$ & $59.087$ & $3.823$ & $4.189$ & $12302$ & $55$ & $49$ \\
SN\,2023bee & HV Si & $59985.6$ & $-6.7$ & $4.580$ & $1.045$ & $1.759$ & $19908$ & $373$ & $352$ \\
SN\,2023bee & C & $59987.5$ & $-4.8$ & $0.206$ & $0.069$ & $0.069$ & \nodata & \nodata & \nodata \\
SN\,2023bee & Si & $59987.5$ & $-4.8$ & $59.349$ & $2.176$ & $1.395$ & $11804$ & $27$ & $26$ \\
SN\,2023bee & HV Si & $59987.5$ & $-4.8$ & $1.260$ & $1.313$ & $0.411$ & $19758$ & $730$ & $340$ \\
SN\,2023bee & C & $59990.5$ & $-1.8$ & $0.147$ & $0.049$ & $0.049$ & \nodata & \nodata & \nodata \\
SN\,2023bee & Si & $59990.5$ & $-1.8$ & $59.010$ & $1.297$ & $2.911$ & $11438$ & $34$ & $41$ \\
SN\,2023bee & C & $59991.5$ & $-0.8$ & $0.200$ & $0.067$ & $0.067$ & \nodata & \nodata & \nodata \\
SN\,2023bee & Si & $59991.5$ & $-0.8$ & $58.668$ & $3.166$ & $5.648$ & $11644$ & $84$ & $58$ \\
SN\,2023wrk & C & $60253.9$ & $-15.2$ & $16.414$ & $5.128$ & $5.258$ & $18909$ & $390$ & $355$ \\
SN\,2023wrk & C & $60254.9$ & $-14.3$ & $21.505$ & $8.714$ & $6.097$ & $19033$ & $813$ & $728$ \\
SN\,2023wrk & Si & $60254.9$ & $-14.3$ & $15.418$ & $8.495$ & $5.650$ & $17448$ & $396$ & $318$ \\
SN\,2023wrk & C & $60255.9$ & $-13.3$ & $7.313$ & $3.367$ & $3.017$ & $16982$ & $485$ & $495$ \\
SN\,2023wrk & Si & $60255.9$ & $-13.3$ & $28.308$ & $10.938$ & $7.278$ & $15638$ & $479$ & $414$ \\
SN\,2023wrk & C & $60256.9$ & $-12.3$ & $3.264$ & $3.791$ & $1.952$ & $15640$ & $573$ & $575$ \\
SN\,2023wrk & Si & $60256.9$ & $-12.3$ & $36.889$ & $5.532$ & $5.772$ & $15396$ & $272$ & $250$ \\
SN\,2023wrk & C & $60257.5$ & $-11.7$ & $2.769$ & $0.572$ & $0.618$ & $16121$ & $135$ & $135$ \\
SN\,2023wrk & Si & $60257.5$ & $-11.7$ & $27.503$ & $2.957$ & $4.000$ & $15030$ & $119$ & $148$ \\
SN\,2023wrk & C & $60258.5$ & $-10.8$ & $2.173$ & $0.445$ & $1.736$ & $15711$ & $596$ & $128$ \\
SN\,2023wrk & Si & $60258.5$ & $-10.8$ & $27.278$ & $2.291$ & $3.374$ & $14972$ & $115$ & $107$ \\
SN\,2023wrk & C & $60259.2$ & $-10.1$ & $0.436$ & $0.145$ & $0.145$ & \nodata & \nodata & \nodata \\
SN\,2023wrk & Si & $60259.2$ & $-10.1$ & $31.289$ & $3.838$ & $2.609$ & $14284$ & $190$ & $160$ \\
SN\,2023wrk & C & $60260.9$ & $-8.4$ & $0.475$ & $0.158$ & $0.158$ & \nodata & \nodata & \nodata \\
SN\,2023wrk & Si & $60260.9$ & $-8.4$ & $32.728$ & $3.609$ & $3.631$ & $14057$ & $145$ & $135$ \\
SN\,2023wrk & C & $60262.9$ & $-6.5$ & $0.202$ & $0.067$ & $0.067$ & \nodata & \nodata & \nodata \\
SN\,2023wrk & Si & $60262.9$ & $-6.5$ & $27.318$ & $2.501$ & $3.813$ & $13787$ & $114$ & $142$ \\
SN\,2023wrk & C & $60263.9$ & $-5.5$ & $0.543$ & $0.181$ & $0.181$ & \nodata & \nodata & \nodata \\
SN\,2023wrk & Si & $60263.9$ & $-5.5$ & $32.080$ & $3.135$ & $4.669$ & $13857$ & $192$ & $132$ \\
SN\,2023wrk & C & $60265.2$ & $-4.2$ & $0.385$ & $0.495$ & $0.343$ & $14139$ & $116$ & $140$ \\
SN\,2023wrk & Si & $60265.2$ & $-4.2$ & $33.915$ & $2.780$ & $7.625$ & $13767$ & $66$ & $70$ \\
SN\,2023wrk & C & $60266.6$ & $-2.8$ & $0.843$ & $0.420$ & $0.614$ & $14111$ & $89$ & $60$ \\
SN\,2023wrk & Si & $60266.6$ & $-2.8$ & $43.103$ & $1.510$ & $2.000$ & $13699$ & $49$ & $33$ \\
SN\,2023wrk & C & $60268.8$ & $-0.7$ & $0.423$ & $1.186$ & $0.333$ & $12770$ & $701$ & $939$ \\
SN\,2023wrk & Si & $60268.8$ & $-0.7$ & $47.547$ & $2.762$ & $2.854$ & $13808$ & $45$ & $43$ \\
SN\,2024epr & C & $60389.8$ & $-16.7$ & $1.547$ & $0.583$ & $0.879$ & $14644$ & $90$ & $61$ \\
SN\,2024epr & Si & $60389.8$ & $-16.7$ & $128.418$ & $5.809$ & $16.378$ & $18462$ & $87$ & $130$ \\
SN\,2024epr & HV Si & $60389.8$ & $-16.7$ & $16.584$ & $2.244$ & $4.509$ & $30249$ & $430$ & $362$ \\
SN\,2024epr & C & $60391.2$ & $-15.3$ & $0.967$ & $0.322$ & $0.322$ & \nodata & \nodata & \nodata \\
SN\,2024epr & Si & $60391.2$ & $-15.3$ & $144.051$ & $8.015$ & $7.375$ & $17135$ & $71$ & $84$ \\
SN\,2024epr & HV Si & $60391.2$ & $-15.3$ & $8.286$ & $8.559$ & $4.192$ & $28052$ & $758$ & $237$ \\
SN\,2024epr & C & $60393.0$ & $-13.5$ & $0.636$ & $0.212$ & $0.212$ & \nodata & \nodata & \nodata \\
SN\,2024epr & Si & $60393.0$ & $-13.5$ & $151.453$ & $5.005$ & $4.431$ & $16429$ & $49$ & $48$ \\
SN\,2024epr & HV Si & $60393.0$ & $-13.5$ & $9.984$ & $2.046$ & $2.445$ & $28119$ & $249$ & $228$ \\
SN\,2024epr & C & $60396.2$ & $-10.3$ & $0.541$ & $0.180$ & $0.180$ & \nodata & \nodata & \nodata \\
SN\,2024epr & Si & $60396.2$ & $-10.3$ & $154.571$ & $3.461$ & $4.696$ & $14500$ & $45$ & $50$ \\
SN\,2024epr & C & $60406.2$ & $-0.4$ & $0.685$ & $0.228$ & $0.228$ & \nodata & \nodata & \nodata \\
SN\,2024epr & Si & $60406.2$ & $-0.4$ & $171.854$ & $3.765$ & $8.888$ & $11723$ & $55$ & $92$ \\
\hline
\end{tabular}
\end{table*}

